Large Skew-t Copula Models and Asymmetric Dependence in Intraday Equity Returns

Skew-t copula models are attractive for the modeling of financial data because they allow for asymmetric and extreme tail dependence. We show that the copula implicit in the skew-t distribution of Azzalini and Capitanio (2003) allows for a higher level of pairwise asymmetric dependence than two popular alternative skew-t copulas. Estimation of this copula in high dimensions is challenging, and we propose a fast and accurate Bayesian variational inference (VI) approach to do so. The method uses a generative representation of the skew-t distribution to define an augmented posterior that can be approximated accurately. A stochastic gradient ascent algorithm is used to solve the variational optimization. The methodology is used to estimate skew-t factor copula models with up to 15 factors for intraday returns from 2017 to 2021 on 93 U.S. equities. The copula captures substantial heterogeneity in asymmetric dependence over equity pairs, in addition to the variability in pairwise correlations. In a moving window study we show that the asymmetric dependencies also vary over time, and that intraday predictive densities from the skew-t copula are more accurate than those from benchmark copula models. Portfolio selection strategies based on the estimated pairwise asymmetric dependencies improve performance relative to the index.

==> acknowl.tex <==

\vspace{0.75em}
\noindent{\large {\bf Acknowledgments}}\\
Nadja Klein gratefully acknowledges funding from the German Alexander von Humboldt foundation. We thank
MutualArt for providing the print price data. 


==> figs.tex <==

\begin{figure}[!thb]
	\caption{Marginals of Different Gaussian Copula Model VAs}
	\begin{center}
		\includegraphics*[scale = 0.7]{figs/densities.eps}
	\end{center}
	Marginal densities $q_i^{\mbox{\tiny SLN2020}}$ (yellow line) and $q_{\lambda_i}$ at~\eqref{eq:EVAmargin} (red line) of optimal VAs
	to two skew normal (SN) target densities (blue line). Both target distributions have 
	the same Pearson skew of 0.8553 and standard deviation $\sigma_{SN}=1$. 
	Panel~(a) plots VA densities when the target mean is $\mu_{SN}=15$, and
	panel~(b) plots VA densities when the target mean is $\mu_{SN}=0$. Also 
	reported are the KL divergences for the optimal approximations.
	\label{fig:KLmargin}
\end{figure}

\begin{figure}[!tb]
	\caption{Kullback-Leibler Divergence of Gaussian Copula Model VA Marginals}
	\begin{center}
		\includegraphics*[scale = 0.8]{figs/Surface.eps}
	\end{center}
	KL divergence of optimal marginal approximations to SN target densities. 
	The SN distributions have a Pearson skew of 0.8553, but different means $\mu_{SN}$ and standard
	deviations $\sigma_{SN}$. Gaussian approximations have KL divergence
	of 0.172 for all target densities (black dashed line), and the approximation $q_{\lambda_i}$ at~\eqref{eq:EVAmargin} has KL divergence of 0.009 for all target densities (solid black line). The KL divergence of $q_i^{\mbox{\tiny SLN2020}}$ is plotted as curves for four values of $\sigma_{SN}$ and $0<\mu_{SN}<60$. 
	The two cases corresponding to Figure~\ref{fig:KLmargin}(a,b) are indicated with circles.
	\label{fig:KLSN}
\end{figure}

\begin{figure}[!tb]
	\caption{Accuracy of Posterior Moments for Mixed Logistic Regression Example}
	\begin{center}
		\includegraphics*[trim = 3cm 1cm 3cm 1cm,clip,width=\textwidth]{figs/Polypharm_moments.eps}
	\end{center}
Panels (a)--(c) are for the t-copula model VA proposed here, and panels~(d)--(f) are for the Gaussian copula model VA in~\cite{smith2020trans}.
In each panel the exact posterior moment (computed using MCMC) is plotted on the horizontal axis, 
and moment of the VA on the vertical axis. The posterior means, standard deviations and Pearson's skew are plotted in the first, second and third columns, respectively. 
In each panel there is a scatter of $m=509$ 
points for each of three variational estimators that correspond to the YJ (blue circles),
iGH (red cross) and YJ-Double (yellow square) transformations for $t_{\gamma_i}$.
For panels~(a)--(e), the results
are very similar for the three transformations, so that most points are close to each other and hard to distinguish.
	\label{fig:polymoments}
\end{figure}

\begin{figure}[!tb]
	\caption{Posteriors for Three Random Effects in the Mixed Logistic Regression Example}
	\begin{center}
		\includegraphics*[trim = 3cm 0cm 3cm 0cm, clip, width=\textwidth]{figs/RE_densities.eps}
	\end{center}
Marginal posterior densities for three random effects.  Each panel plots the exact posterior
computed by MCMC (black line), the t-copula model VA $q_{\lambda_i}$ at~\eqref{eq:qmargin} (red line) and that in~\cite{smith2020trans} $q_i^{\mbox{\tiny SLN2020}}$ (yellow line), both using the iGH transformation. 
	\label{fig:polyRE}
\end{figure}

\begin{figure}[!p]
	\caption{Exact Posterior for the Two U.S. States Inequality Example}
	\begin{center}
		\includegraphics*[width=\textwidth]{figs/CATX_mcmc.eps}
	\end{center}
	Exact posterior of $(\theta_1,\ldots,\theta_5)^\top=(\tau_1,\log \chi_1, \log \nu_1, \log \xi, \log \kappa)^\top$ computed using MCMC. The univariate marginals $p(\theta_i|\yvec)$ are on the leading diagonals, and 
	the bivariate marginals $p(\theta_i,\theta_j|\yvec)$ are on the off-diagonals. 
	\label{fig:CATX_mcmc}
\end{figure}

\begin{figure}[!p]
	\caption{Variational Posterior for the Two U.S. States Inequality Example}
	\begin{center}
		\includegraphics*[width=\textwidth]{figs/CATX_copVA.eps}
	\end{center}
	Posterior estimates of $(\theta_1,\ldots,\theta_5)^\top=(\tau_1,\log \chi_1, \log \nu_1, \log \xi, \log \kappa)^\top$
	using the copula model VA with (adjusted) YJ transformations. 
	The marginals $q_{\lambda_i}(\theta_i)$ are on the leading diagonals, and 
	the bivariate marginals---which are bivariate slices of~\eqref{Eq:VA}---are on the off-diagonals. 
	\label{fig:CATX_copVA}
\end{figure}

\begin{figure}[!tbhp]
	\caption{Variational Posterior Densities of Spearman Correlations for Five Western States}
	\begin{center}
		\includegraphics*[width=0.7\textwidth]{figs/west_spear.eps}
	\end{center}
Variational posterior densities of the 10 Spearman correlations between the contiguous western U.S. states of WA, OR, CA, NV and AZ. The posterior for the
more accurate optimal t-copula is in blue, while that from the mean field t-distribution is in black. 
	\label{fig:west_spear}
\end{figure}


==> tabs.tex <==
\begin{table}[htb]
	\begin{center}
	\small%\renewcommand\arraystretch{1.15}
	\caption{Point forecast accuracy of models during the evaluation period}\label{tab:pointfore}
	\begin{tabular}{llllllll}
		\hline
		&\multicolumn{7}{c}{Hours Ahead in the Forecast Horizon}\\ \cline{2-8}
		Model & 0.5 hour & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
		\hline
		&\multicolumn{7}{l}{MAE}\\ \cline{2-8}
GAMLSS & 0.0226$^{***}$ & 0.0314$^{***}$ & 0.0408$^{***}$ & 0.0468$^{***}$ & 0.0591$^{***}$ & 0.0692$^{***}$ & 0.0766$^{***}$ \\ 
  RNN & 0.0249$^{***}$ & 0.0319$^{***}$ & 0.0411$^{***}$ & 0.0494$^{***}$ & 0.0600$^{***}$ & 0.0722$^{***}$ & 0.0800$^{***}$ \\ 
  RNNSN & 0.0221$^{***}$ & 0.0219$^{*}$ & 0.0239 & 0.0252 & 0.0262 & 0.0268$^{**}$ & 0.0278$^{***}$ \\ 
  RNNST & 0.0189 & 0.0210 & 0.0231 & 0.0242 & 0.0250 & 0.0255$^{***}$ & 0.0257$^{***}$ \\ 
 \emph{RNNC}& \emph{0.0169} & \emph{0.0194} & \emph{0.0224} & \emph{0.0238} & \emph{0.0252} & \emph{0.0244} & \emph{0.0239} \\ 
 
		&\multicolumn{7}{l}{RMSE}\\ \cline{2-8}
GAMLSS & 0.0340$^{\mbox{\tiny{+}}}$ & 0.0461$^{\mbox{\tiny{++}}}$ & 0.0610$^{\mbox{\tiny{+++}}}$ & 0.0623$^{\mbox{\tiny{+++}}}$ & 0.0644$^{\mbox{\tiny{+++}}}$ & 0.0653 & 0.0661 \\ 
  RNN & 0.0537 & 0.0616$^{\mbox{\tiny{**}}}$ & 0.0712 & 0.0797 & 0.0935 & 3.7173$^{***}$  & 16.5496$^{***}$  \\ 
  RNNSN & 0.0538 & 0.0572 & 0.0603 & 0.0615 & 0.0623 & 0.0629 & 0.0638 \\ 
  RNNST & 0.0528$^{\mbox{\tiny{+}}}$ & 0.0571 & 0.0603 & 0.0612 & 0.0623 & 0.0630 & 0.0635 \\ 
  \emph{RNNC} & \emph{0.0538 }& \emph{0.0573 }&\emph{ 0.0613} & \emph{0.0638} & \emph{0.0657} & \emph{0.0632} & \emph{0.0629} \\ 
  
%GAMLSS & 0.0455 & 0.0485 & 0.0494 & 0.0480 & 0.0471 & 0.0475 \\ 
%  RNN & 0.0503$^{\mbox{\tiny{+++}}}$ & 0.0507 & 0.0511 & 0.0520 & 0.0535 & 0.0565 \\ 
%  RNNSN & 0.0491 & 0.0485 & 0.0494 & 0.0482 & 0.0492 & 0.0489 \\ 
%  RNNST & 0.0478 & 0.0473 & 0.0474 & 0.0471 & 0.0471 & 0.0474 \\ 
%  {\em RNNC} & {\em 0.0529} & {\em 0.0547} & {\em 0.0542} & {\em 0.0567} & {\em 0.0511} & {\em 0.0486} \\ 
		\hline
	\end{tabular}
\end{center}
		Both the system-weighted mean absolute error (MAE) and root
		mean squared error (RMSE) are reported. Results are given for the four deep time series models, plus GAMLSS. Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC with each of the other models are reported. Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC model, or by ``${\mbox{\tiny{+}}}$'', ``${\mbox{\tiny{++}}}$'' and
		``${\mbox{\tiny{+++}}}$'' if unfavorable.
\end{table}

\begin{table}[ht]
\begin{center}
\caption{Probabilistic forecast accuracy during the evaluation period.}\label{tab:densityfore}
\centering\small%\renewcommand\arraystretch{1.25}
\begin{tabular}{lllllllll}
  \hline
		&\multicolumn{7}{c}{Hours Ahead in the Forecast Horizon}\\ \cline{2-8}
		Model & 0.5 hour & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours  \\ \hline
  &\multicolumn{7}{l}{{\em CRPS}}\\ \cline{2-8}
GAMLSS & 0.0180$^{***}$ & 0.0252$^{***}$ & 0.0335$^{***}$ & 0.0392$^{***}$ & 0.0508$^{***}$ & 0.0601$^{***}$ & 0.0652$^{***}$ \\ 
  RNN & 0.0203$^{***}$ & 0.0235$^{***}$ & 0.0299$^{***}$ & 0.0364$^{***}$ & 0.0449$^{***}$ & 0.0574$^{***}$ & 0.4061$^{***}$ \\ 
  RNNSN & 0.0174$^{***}$ & 0.0177$^{**}$ & 0.0191 & 0.0201 & 0.0207 & 0.0212$^{**}$ & 0.0219$^{***}$ \\ 
  RNNST & 0.0157$^{***}$ & 0.0172$^{***}$ & 0.0187$^{***}$ & 0.0195 & 0.0201 & 0.0206$^{***}$ & 0.0208$^{***}$ \\
 \emph{RNNC} & \emph{0.0135} & \emph{0.0154} & \emph{0.0177} & \emph{0.0189} & \emph{0.0199} & \emph{0.0193} & \emph{0.0187} \\ 
  &\multicolumn{6}{l}{{\em Joint Upper Tail Loss at }$\alpha=0.975$}\\ \cline{2-8}
GAMLSS & 31.6394$^{*}$ & 32.4717$^{***}$ & 33.2367$^{***}$ & 33.9396$^{***}$ & 35.9352$^{***}$ & 40.0541$^{***}$ & 39.7960$^{***}$ \\ 
  RNN & 30.8568 & 31.5025 & 33.3171 & 35.5605 & 39.2732$^{**}$ & 41.9374$^{***}$ & 33.4037$^{***}$ \\ 
  RNNSN & 32.1052$^{**}$ & 31.2797 & 31.6342 & 31.6492 & 31.7099 & 31.5852$^{***}$ & 31.3780$^{***}$ \\ 
  RNNST & 31.3493$^{*}$ & 31.4414 & 31.6911 & 32.0056$^{*}$ & 31.8607 & 32.2372$^{***}$ & 31.8694$^{***}$ \\ 
  \emph{RNNC} & \emph{30.1002} & \emph{30.6244} & \emph{31.0090} & \emph{31.0934} & \emph{31.1121} & \emph{30.6238} & \emph{29.7661} \\ 
  
&\multicolumn{7}{l}{{\em Quantile Score at} $\alpha=0.95$}\\ \cline{2-8}
GAMLSS & 0.0056$^{***}$ & 0.0069$^{***}$ & 0.0082$^{***}$ & 0.0093$^{***}$ & 0.0124$^{***}$ & 0.0190$^{***}$ & 0.0198$^{***}$ \\ 
  RNN & 0.0050 & 0.0057 & 0.0078$^{***}$ & 0.0107$^{***}$ & 0.0155$^{***}$ & 0.0201$^{***}$ & 1.0808$^{***}$ \\ 
  RNNSN & 0.0056 & 0.0050 & 0.0054 & 0.0055 & 0.0057 & 0.0058$^{*}$ & 0.0060$^{***}$ \\ 
  RNNST & 0.0048 & 0.0050 & 0.0054 & 0.0057$^{**}$ & 0.0057$^{*}$ & 0.0062$^{***}$ & 0.0063$^{***}$ \\ 
  \emph{RNNC} & \emph{0.0036} & \emph{0.0043} & \emph{0.0048} & \emph{0.0050} & \emph{0.0052} & \emph{0.0050} & \emph{0.0046} \\ 
  
 &\multicolumn{7}{l}{{\em Quantile Score at} $\alpha=0.05$}\\ \cline{2-8}
 
GAMLSS & 0.0049$^{***}$ & 0.0080$^{***}$ & 0.0129$^{***}$ & 0.0167$^{***}$ & 0.0242$^{***}$ & 0.0260$^{***}$ & 0.0298$^{***}$ \\ 
  RNN & 0.0047 & 0.0053 & 0.0057$^{***}$ & 0.0061 & 0.0069$^{***}$ & 0.0096$^{***}$ & 0.5602$^{***}$ \\ 
  RNNSN & 0.0046$^{**}$ & 0.0055 & 0.0056 & 0.0062 & 0.0061 & 0.0064 & 0.0065 \\ 
  RNNST & 0.0048$^{***}$ & 0.0055$^{*}$ & 0.0059$^{**}$ & 0.0061 & 0.0064 & 0.0063 & 0.0066 \\ 
  \emph{RNNC} & \emph{0.0039} & \emph{0.0046} & \emph{0.0053} & \emph{0.0058} & \emph{0.0061} & \emph{0.0059} & \emph{0.0057} \\  
  \hline
\end{tabular}
\end{center}
System-weighted metrics are reported for the four deep time series models, plus
GAMLSS, at different points in time during a 24 hour forecast horizon. 
Lower values suggest greater accuracy. Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC with each of the other models are reported.
Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC model, or by ``${\mbox{\tiny{+}}}$'', ``${\mbox{\tiny{++}}}$'' and
``${\mbox{\tiny{+++}}}$'' if unfavorable.
\end{table}

%
%\begin{table}[ht]
%\centering\small\renewcommand\arraystretch{1.25}
%\begin{tabular}{c|cccccc}
%  \hline
%Method & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
%  \hline
%RNNC & 0.0472 & 0.0489 & 0.0495 & 0.0525 & 0.0476 & 0.0450 \\ 
%  GAMLSS & 0.0527 & 0.1123 & 0.1013 & 0.1015 & 0.1428 & 0.1975 \\ 
%  RNNST & 0.0419 & 0.0421 & 0.0427 & 0.0429 & 0.0428 & 0.0431 \\ 
%  RNNSN & 0.0440 & 0.0437 & 0.0453 & 0.0441 & 0.0451 & 0.0452 \\ 
%  RNN & 0.0440 & 0.0450 & 0.0457 & 0.0468 & 0.0480 & 0.0504 \\ 
%   \hline
%\end{tabular}
% \caption{System weighted RMSE values computed from the simulated ahead forecast values.
% 	Results from all three models are shown, these are RNNC, GAMLSS, RNNSN, RNN. Lower values correspond to higher predictive accuracy. The system weights are: NSW: 0.3687
%VIC: 0.2355
%QLD: 0.2818
%TAS: 0.0516
%SA: 0.0624. }\label{tab:RNN:RMSE}
%\end{table}

%
%\begin{table}[ht]
%\centering\small\renewcommand\arraystretch{1.25}
%\begin{tabular}{c|cccccc}
%  \hline
%Method & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
%  \hline
%RNNC & 32.5610 & 32.9776 & 33.1809 & 33.8470 & 32.8989 & 31.7415 \\ 
%  GAMLSS & 33.5579 & 34.5999 & 39.7815 & 46.3045 & 71.7834 & 305.0956 \\ 
%  RNNST & 33.2465 & 33.5892 & 33.7738 & 33.8191 & 33.7791 & 34.0819 \\ 
%  RNNSN & 36.6275 & 36.4510 & 36.3765 & 35.8254 & 37.7442 & 36.9532 \\ 
%  RNN & 34.1640 & 34.4068 & 34.5347 & 34.6406 & 34.7903 & 35.0608 \\  
%   \hline
%\end{tabular}
% \caption{System weighted joint score computed from the simulated ahead forecast values for $\alpha=0.975$.
% 	Results from all three models are shown, these are RNNC, GAMLSS, RNNSN, RNN. Lower values correspond to higher predictive accuracy. The system weights are: NSW: 0.3687
%VIC: 0.2355
%QLD: 0.2818
%TAS: 0.0516
%SA: 0.0624. }\label{tab:RNN:JS}
%\end{table}


%\begin{table}[ht]
%\centering\small\renewcommand\arraystretch{1.25}
%\begin{tabular}{c|cccccc}
%  \hline
%Method & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours \\ 
%  \hline
%RNNC & 0.0089 & 0.0092 & 0.0093 & 0.0095 & 0.0091 & 0.0089 \\ 
%  GAMLSS & 0.0093 & 0.0113 & 0.0118 & 0.0141 & 0.0196 & 0.0317 \\ 
%  RNNST & 0.0086 & 0.0087 & 0.0088 & 0.0088 & 0.0088 & 0.0089 \\ 
%  RNNSN & 0.0105 & 0.0107 & 0.0113 & 0.0109 & 0.0112 & 0.0113 \\ 
%  RNN & 0.0140 & 0.0141 & 0.0142 & 0.0146 & 0.0148 & 0.0155 \\ 
%   \hline
%\end{tabular}
% \caption{System weighted mean quantile score computed from the simulated ahead forecast values.
% 	Results from all three models are shown, these are RNNC, GAMLSS, RNNSN, RNN. Lower values correspond to higher predictive accuracy. The system weights are: NSW: 0.3687
%VIC: 0.2355
%QLD: 0.2818
%TAS: 0.0516
%SA: 0.0624. }\label{tab:RNN:QS}
%\end{table}

\begin{table}[ht]
\begin{center}
\centering\small\renewcommand\arraystretch{1.25}
 \caption{Coverage of 95\% prediction intervals during the 
	evaluation period.}\label{tab:RNN:covs}
\begin{tabular}{lccccccc}
  \hline
		&\multicolumn{7}{c}{Hours Ahead in the Forecast Horizon}\\ \cline{2-8}
		Model & 0.5 hour & 1 hour & 2 hours & 3 hours & 6 hours & 12 hours & 24 hours  \\ \hline
GAMLSS & 0.9078 & 0.8148 & 0.7278 & 0.6928 & 0.6476 & 0.5838 & 0.5208 \\ 
  RNN & 0.8715 & 0.8609 & 0.7906 & 0.7173 & 0.6336 & 0.5698 & 0.6124 \\ 
  RNNSN & 0.8496 & 0.8386 & 0.8354 & 0.8187 & 0.8123 & 0.7998 & 0.7759 \\ 
  RNNST & 0.8550 & 0.8424 & 0.8353 & 0.8216 & 0.8171 & 0.7955 & 0.7667 \\ 
  \emph{RNNC} & \emph{0.9279} & \emph{0.9012} & \emph{0.8791} & \emph{0.8741} & \emph{0.8620} & \emph{0.8594} & \emph{0.8706} \\ 
   \hline
\end{tabular}
\end{center}
  Results are reported
 	for the four deep time series models, plus
 	GAMLSS, at different points in time in the 24 hour forecast horizon.
 	Values closer to 0.95 indicate improved calibration of the probabilistic forecasts.
\end{table}

\begin{table}[htb]
	\begin{center}
\centering\small\renewcommand\arraystretch{1.25}
 \caption{NSW price forecast accuracy when
 	including demand forecast information.} \label{tab:foredemand}
\begin{tabular}{lllllllll}
  \hline\hline
Model &  MAE & RMSE & CRPS & &JS &QS95 & QS05 & C95 \\ 
  \hline
&   \multicolumn{3}{l}{Point and Density Accuracy} &  &\multicolumn{3}{l}{Tail Accuracy} & \\ \cline{2-4} \cline{6-8}
%  &\multicolumn{6}{l}{Without Demand Forecasts as Features}\\ \cline{2-8}
\textit{RNNC+D} & \textit{0.0192 } &  \textit{0.0314}  &  \textit{0.0146} & & \textit{30.6902}  &  \textit{0.0045}   & \textit{0.0025} & 82.6\% \\
RNNC & 0.0188$^{\mbox{\tiny{+++}}}$   & 0.0311$^{\mbox{\tiny{+++}}}$ &  0.0144$^{\mbox{\tiny{+++}}}$ &&  31.0350$^{**}$  &  0.0048$^{***}$    & 0.0023 & 84.5\% \\   
%  &\multicolumn{6}{l}{Including Demand Forecasts as Features}\\ \cline{2-8}
%  RNNCcov & 0.0115 & 0.0313 & 0.0143 & 30.4646 & 0.0069 & \textbf{0.8390} \\ 
%  RNNSTcov   & 0.0147 & 0.0316 & 0.0160 & 31.8385 & 0.0078 & 0.8128 \\ 
 RNNST &0.0250$^{***}$    &0.0401    &0.0221$^{***}$ &  &39.4411$^{***}$    &0.0121$^{***}$    &0.0049$^{***}$ & 46.2 \%\\
  RNNST+D & 0.0256$^{***}$ &   0.0395  &  0.0222$^{***}$ && 39.6431$^{***}$   & 0.0123$^{***}$  &  0.0046$^{***}$ & 53.9\% \\ 
   \hline\hline
\end{tabular}
\end{center}
 Accuracy of 24 hour ahead NSW (logarithmic) price forecasts during the evaluation period. Models that include 24 hour ahead demand forecast information as features are labelled as ``+D''. The metrics are described in the text, and
include the joint score (JS) at $\alpha=0.975$, quantile score (QS) at $\alpha=0.95,0.05$, and the empirical coverage of the 95\% prediction intervals (C95). %The stars ``*'', ``**'' ,``***'' at RNNC+D indicate significantly better metrics for RNNC+D than for RNNC at the $1,5,10\%$ levels using a two-sided Diebold-Marino (DM) test statistic. Similarly for RNNST+D and RNNST+D.
Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC+D with the other methods are reported. Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC+D model, or by ``${\mbox{\tiny{+}}}$'', ``${\mbox{\tiny{++}}}$'' and ``${\mbox{\tiny{+++}}}$'' if unfavorable.
\end{table}



%Results of a two-sided Diebold-Mariano test of the equality of the mean error of the RNNC with each of the other models are reported. Rejection of the null hypothesis of equal means at the 10\%, 5\% and 1\% levels are denoted by ``*'', ``**'' and ``***'' if favorable to the RNNC model, or by ``${\mbox{\tiny{+}}}$'', %``${\mbox{\tiny{++}}}$'' and
%		``${\mbox{\tiny{+++}}}$'' if unfavorable.

